A Stronger Baseline For Automatic Pfirrmann Grading Of Lumbar Spine MRI Using Deep Learning

This paper addresses the challenge of grading visual features in lumbar spine MRI using Deep Learning. Such a method is essential for the automatic quantification of structural changes in the spine, which is valuable for understanding low back pain. Multiple recent studies investigated different architecture designs, and the most recent success has been attributed to the use of transformer architectures. In this work, we argue that with a well-tuned three-stage pipeline comprising semantic segmentation, localization, and classification, convolutional networks outperform the state-of-the-art approaches. We conducted an ablation study of the existing methods in a population cohort, and report performance generalization across various subgroups. Our code is publicly available to advance research on disc degeneration and low back pain.

==> tab_subgroups.tex <==
\begin{table}[ht!]
\caption{Performance of the model along different intervertebral discs, sex, LBP, and Pfirrmann grades (in BA, \%).}
\label{tbl:subgroups}
\resizebox{\linewidth}{!}{
\begin{tabular}{rlccccc}
\toprule
\multicolumn{1}{l}{Parameter} &                      & \multicolumn{5}{c}{Intervertebral Disc Level}                            \\ \midrule
\multicolumn{1}{l}{}& \multicolumn{1}{c}{} & L1-L2  & L2-L3  & L3-L4  & L4-L5  & L5-S1 \\ \midrule
\multicolumn{7}{l}{Sex}\\ 
\multicolumn{2}{r}{Male}                   & $73.3$ & $83.4$ & $76.4$ & $82.7$ & $83.1$ \\ 
\multicolumn{2}{r}{Female}                 & $79.4$ & $77.8$ & $65.8$ & $76.7$ & $80.8$  \\ 
\midrule
\multicolumn{7}{l}{With LBP}\\ 
\multicolumn{2}{r}{Male}                   & $58.4$ & $83.4$ & $85.3$ & $84.1$ & $83.3$\\
\multicolumn{2}{r}{Female}                 & $83.8$ & $77.8$ & $67.4$ & $78.9$ & $80.5$\\ 
\multicolumn{2}{r}{Pain ($<30$ Days)}      & $66.7$ & $78.3$ & $72.2$ & $82.1$ & $82.4$\\
\multicolumn{2}{r}{Prolonged LBP}          & $84.6$ & $87.6$ & $77.9$ & $81.0$ & $82.7$\\ 
\midrule
\multicolumn{7}{l}{Pfirrmann grade}\\
\multicolumn{2}{r}{Grade 2}                & $94.2$ & $92.4$ & $85.6$ & $80.6$ & $88.4$\\
\multicolumn{2}{r}{Grade 3}                & $68.6$ & $71.7$ & $78.8$ & $76.4$ & $75.2$\\
\multicolumn{2}{r}{Grade 4}                & $72.5$ & $71.8$ & $71.9$ & $77.8$ & $81.6$\\
\multicolumn{2}{r}{Grade 5}                & $68.1$ & $88.0$ & $53.1$ & $91.4$ & $85.0$ \\ 
\bottomrule
\end{tabular}
}
\end{table}
